Constraint Preconditioning and Parameter Selection for a First-Order Primal-Dual Method applied to Model Predictive Control

Many techniques for real-time trajectory optimization and control require the solution of optimization problems at high frequencies. However, ill-conditioning in the optimization problem can significantly reduce the speed of first-order primal-dual optimization algorithms. We introduce a preconditioning technique and step-size heuristic for Proportional-Integral Projected Gradient (PIPG), a first-order primal-dual algorithm. The preconditioning technique, based on the QR factorization, aims to reduce the condition number of the KKT matrix associated with the optimization problem. Our step-size selection heuristic chooses step-sizes to minimize the upper bound on the convergence of the primal-dual gap for the optimization problem. These algorithms are tested on two model predictive control problem examples and show a solve-time reduction of at least 3.6x.

==> sections/2-notation.tex <==
\section{NOTATION}
We denote the $n \times n$ square matrix of zeros as $0_n$, the $m \times n$ matrix of zeros as $0_{m \times n}$, the $n \times n$ identity matrix as $I_n$, the Euclidean projection of point $z$ onto the convex set $\mb{D}$ as $\Pi_{\mb{D}}[z]$, the concatenation of vectors $u$ and $v$ as $(u,v)$, the vector formed from the $i^{th}$ through the $j^{th}$ component of $z$ as $z^{i:j}$, and the Euclidean norm of a vector $z$ as $\|z\| := \sqrt{z^\top z}$.

